SEINE: Short-to-Long Video Diffusion Model for Generative Transition and Prediction

Recently video generation has achieved substantial progress with realistic results. Nevertheless, existing AI-generated videos are usually very short clips ("shot-level") depicting a single scene. To deliver a coherent long video ("story-level"), it is desirable to have creative transition and prediction effects across different clips. This paper presents a short-to-long video diffusion model, SEINE, that focuses on generative transition and prediction. The goal is to generate high-quality long videos with smooth and creative transitions between scenes and varying lengths of shot-level videos. Specifically, we propose a random-mask video diffusion model to automatically generate transitions based on textual descriptions. By providing the images of different scenes as inputs, combined with text-based control, our model generates transition videos that ensure coherence and visual quality. Furthermore, the model can be readily extended to various tasks such as image-to-video animation and autoregressive video prediction. To conduct a comprehensive evaluation of this new generative task, we propose three assessing criteria for smooth and creative transition: temporal consistency, semantic similarity, and video-text semantic alignment. Extensive experiments validate the effectiveness of our approach over existing methods for generative transition and prediction, enabling the creation of story-level long videos. Project page: https://vchitect.github.io/SEINE-project/ .

==> sections/discussion.tex <==
\section{Discussion}
While our method excels in transition generation, it does have limitations regarding the similarity of the source and target scenes. This requirement arises from the nature of the transition process, as it relies on finding meaningful correspondences between the two scenes to create a smooth and visually coherent transition. If the scenes are too dissimilar or lack common elements, the transition may appear abrupt or visually inconsistent. 
This limitation can be addressed through a multi-step approach. We can employ image editing techniques to modify the source image to the target image of the scenes and actions. This method is particularly beneficial in scene generation as it operates at the image level, naturally preserving similarities such as the structure, background, and objects of the image. As a result, the transition effects produced using this approach often appear highly natural.
